Comparison of \nu\mu-Ar multiplicity distributions observed by MicroBooNE to GENIE model predictions

We measure a large set of observables in inclusive charged current muon neutrino scattering on argon with the MicroBooNE liquid argon time projection chamber operating at Fermilab. We evaluate three neutrino interaction models based on the widely used GENIE event generator using these observables. The measurement uses a data set consisting of neutrino interactions with a final state muon candidate fully contained within the MicroBooNE detector. These data were collected in 2016 with the Fermilab Booster Neutrino Beam, which has an average neutrino energy of 800 MeV, using an exposure corresponding to 5E19 protons-on-target. The analysis employs fully automatic event selection and charged particle track reconstruction and uses a data-driven technique to separate neutrino interactions from cosmic ray background events. We find that GENIE models consistently describe the shapes of a large number of kinematic distributions for fixed observed multiplicity.

==> author_list.tex <==
%\documentclass[a4paper,11pt]{article}
%\pdfoutput=1 
%\usepackage{jinstpub} 

%\title{MicroBooNE Author List - December 2017 (JINST format)}
%\collaboration{MicroBooNE Collaboration}
%\begin{document}

% make sure the \maketitle command appears AFTER the affiliations!

% For signal processing paper #1 (Jan 2018), add invited authors: Veljko Radeka, Bo Yu, Craig Thorn, Bo Yu
% December 2017: see notes in docdb #13001
% July 2017 MuCS: add Harvard, joint affiliations for Adams, Guenette, Terao
% For Noise paper (Apr 2017), add invited authors: B. Bullard, G. De Geronimo, S. Li, V. Radeka, S. Rescia, C. Thorn, B. Yu
% For MuCS paper (Mar 2017), add invited authors: L.N. Kalousis, G. Lange, R. Pelkey
% For MCS paper (Feb 2017), add invited authors: L.N. Kalousis, P. Abratenko

\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}
\affiliation{University of Cincinnati, Cincinnati, OH, 45221, USA}
\affiliation{Colorado State University, Fort Collins, CO, 80523, USA}
\affiliation{Columbia University, New York, NY, 10027, USA}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\affiliation{Harvard University, Cambridge, MA 02138, USA}
\affiliation{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\affiliation{Kansas State University (KSU), Manhattan, KS, 66506, USA}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\affiliation{University of Michigan, Ann Arbor, MI, 48109, USA}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\affiliation{Otterbein University, Westerville, OH, 43081, USA}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\affiliation{Saint Mary's University of Minnesota, Winona, MN, 55987, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}
\affiliation{Tel Aviv University, Tel Aviv, Israel, 69978}
\affiliation{University of Tennessee, Knoxville, TN, 37996, USA}
\affiliation{University of Texas, Arlington, TX, 76019, USA}
\affiliation{TUBITAK Space Technologies Research Institute, METU Campus, TR-06800, Ankara, Turkey}
\affiliation{Tufts University, Medford, MA, 02155, USA}
\affiliation{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\affiliation{Yale University, New Haven, CT, 06520, USA}


% Authors in alphabetical order
%\author{P.~Abratenko}   % only for MCS paper!
\author{C.~Adams}
\affiliation{Harvard University, Cambridge, MA 02138, USA}

%\author{M.~Alrashed}
\author{R.~An}
\affiliation{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}

\author{J.~Anthony}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

\author{J.~Asaadi}
\affiliation{University of Texas, Arlington, TX, 76019, USA}

\author{M.~Auger}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{S.~Balasubramanian}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{B.~Baller}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{C.~Barnes}
\affiliation{University of Michigan, Ann Arbor, MI, 48109, USA}

\author{G.~Barr}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}

\author{M.~Bass}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{F.~Bay}
\affiliation{TUBITAK Space Technologies Research Institute, METU Campus, TR-06800, Ankara, Turkey}

\author{A.~Bhat}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}

\author{K.~Bhattacharya}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}

\author{M.~Bishai}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{A.~Blake}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}

\author{T.~Bolton}
%\thanks{Corresponding author}
%\email[Email: ]{bolton@phys.ksu.edu}
\affiliation{Kansas State University (KSU), Manhattan, KS, 66506, USA}

%\author{B.~Bullard}     % only for noise paper!
\author{L.~Camilleri}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{D.~Caratelli}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{R.~Castillo~Fernandez}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{F.~Cavanna}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{G.~Cerati}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{H.~Chen}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{Y.~Chen}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{E.~Church}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}

\author{D.~Cianci}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{E.~Cohen}
\affiliation{Tel Aviv University, Tel Aviv, Israel, 69978}

\author{G.~H.~Collin}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{J.~M.~Conrad}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{M.~Convery}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{L.~Cooper-Troendle}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{J.~I.~Crespo-Anad\'{o}n}
\affiliation{Columbia University, New York, NY, 10027, USA}

%\author{G.~De~Geronimo}   % only for noise paper!
\author{M.~Del~Tutto}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}

\author{D.~Devitt}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}

\author{A.~Diaz}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{S.~Dytman}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}

\author{B.~Eberly}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{A.~Ereditato}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{L.~Escudero Sanchez}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

\author{J.~Esquivel}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}

\author{J.~J~Evans}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{A.~A.~Fadeeva}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{B.~T.~Fleming}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{W.~Foreman}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}

\author{A.~P.~Furmanski}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{D.~Garcia-Gamez}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{G.~T.~Garvey}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}

\author{V.~Genty}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{D.~Goeldi}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{S.~Gollapinni}
\affiliation{University of Tennessee, Knoxville, TN, 37996, USA}

\author{E.~Gramellini}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{H.~Greenlee}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{R.~Grosso}
\affiliation{University of Cincinnati, Cincinnati, OH, 45221, USA}

\author{R.~Guenette}
\affiliation{Harvard University, Cambridge, MA 02138, USA}

\author{P.~Guzowski}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{A.~Hackenburg}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{P.~Hamilton}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}

\author{O.~Hen}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{J.~Hewes}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{C.~Hill}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{J.~Ho}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}

\author{G.~A.~Horton-Smith}
\affiliation{Kansas State University (KSU), Manhattan, KS, 66506, USA}

\author{A.~Hourlier}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{E.-C.~Huang}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}

\author{C.~James}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{J.~Jan~de~Vries}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

\author{L.~Jiang}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}

\author{R.~A.~Johnson}
\affiliation{University of Cincinnati, Cincinnati, OH, 45221, USA}

\author{J.~Joshi}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{H.~Jostlein}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{Y.-J.~Jwa}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{D.~Kaleko}
\affiliation{Columbia University, New York, NY, 10027, USA}

%\author[bb,1]{L.~N.~Kalousis\note{now at: Vrije Universiteit Brussel, 1050 Ixelles, Belgium}} % only for MCS and MuCS papers!
\author{G.~Karagiorgi}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{W.~Ketchum}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{B.~Kirby}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{M.~Kirby}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{T.~Kobilarcik}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{I.~Kreslo}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

%\author{G.~Lange}    % only for MuCS paper!
%\author{S.~Li}   % only for noise paper!
\author{Y.~Li}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{A.~Lister}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}

\author{B.~R.~Littlejohn}
\affiliation{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}

\author{S.~Lockwitz}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{D.~Lorca}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{W.~C.~Louis}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}

\author{M.~Luethi}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{B.~Lundberg}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{X.~Luo}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{A.~Marchionni}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{S.~Marcocci}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{C.~Mariani}
\affiliation{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}

\author{J.~Marshall}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

\author{D.~A.~Martinez~Caicedo}
\affiliation{Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}

\author{A.~Mastbaum}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}

\author{V.~Meddage}
\affiliation{Kansas State University (KSU), Manhattan, KS, 66506, USA}

\author{T.~Mettler}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{T.~Miceli}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}

\author{G.~B.~Mills}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}

\author{A.~Mogan}
\affiliation{University of Tennessee, Knoxville, TN, 37996, USA}

\author{J.~Moon}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{M.~Mooney}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\affiliation{Colorado State University, Fort Collins, CO, 80523, USA}

\author{C.~D.~Moore}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{J.~Mousseau}
\affiliation{University of Michigan, Ann Arbor, MI, 48109, USA}

\author{M.~Murphy}
\affiliation{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}

\author{R.~Murrells}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{D.~Naples}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}

\author{P.~Nienaber}
\affiliation{Saint Mary's University of Minnesota, Winona, MN, 55987, USA}

\author{J.~Nowak}
\affiliation{Lancaster University, Lancaster LA1 4YW, United Kingdom}

\author{O.~Palamara}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{V.~Pandey}
\affiliation{Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}

\author{V.~Paolone}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}

\author{A.~Papadopoulou}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

\author{V.~Papavassiliou}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}

\author{S.~F.~Pate}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}

\author{Z.~Pavlovic}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

%\author{R.~Pelkey}    % only for MuCS paper!
\author{E.~Piasetzky}
\affiliation{Tel Aviv University, Tel Aviv, Israel, 69978}

\author{D.~Porzio}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{G.~Pulliam}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}

\author{X.~Qian}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{J.~L.~Raaf}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

%\author{V.~Radeka}   % only for noise paper, signal processing paper #1
\author{A.~Rafique}
%\thanks{Corresponding author}
%\email[Email: ]{aleena@ksu.edu}
\affiliation{Kansas State University (KSU), Manhattan, KS, 66506, USA}

%\author{S.~Rescia}   % only for noise paper!
\author{L.~Rochester}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{M.~Ross-Lonergan}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{C.~Rudolf~von~Rohr}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{B.~Russell}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{D.~W.~Schmitz}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}

\author{A.~Schukraft}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{W.~Seligman}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{M.~H.~Shaevitz}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{J.~Sinclair}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{A.~Smith}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

\author{E.~L.~Snider}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{M.~Soderberg}
\affiliation{Syracuse University, Syracuse, NY, 13244, USA}

\author{S.~S{\"o}ldner-Rembold}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{S.~R.~Soleti}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}

\author{P.~Spentzouris}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{J.~Spitz}
\affiliation{University of Michigan, Ann Arbor, MI, 48109, USA}

\author{J.~St.~John}
\affiliation{University of Cincinnati, Cincinnati, OH, 45221, USA}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{T.~Strauss}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{K.~Sutton}
\affiliation{Columbia University, New York, NY, 10027, USA}

\author{S.~Sword-Fehlberg}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}

\author{A.~M.~Szelc}
\affiliation{The University of Manchester, Manchester M13 9PL, United Kingdom}

\author{N.~Tagg}
\affiliation{Otterbein University, Westerville, OH, 43081, USA}

\author{W.~Tang}
\affiliation{University of Tennessee, Knoxville, TN, 37996, USA}

\author{K.~Terao}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{M.~Thomson}
\affiliation{University of Cambridge, Cambridge CB3 0HE, United Kingdom}

%\author{C.~Thorn}  % only for noise paper and signal processing paper #1
\author{M.~Toups}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{Y.-T.~Tsai}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{S.~Tufanli}
\affiliation{Yale University, New Haven, CT, 06520, USA}

\author{T.~Usher}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}

\author{W.~Van~De~Pontseele}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}

\author{R.~G.~Van~de~Water}
\affiliation{Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}

\author{B.~Viren}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{M.~Weber}
\affiliation{Universit{\"a}t Bern, Bern CH-3012, Switzerland}

\author{H.~Wei}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}

\author{D.~A.~Wickremasinghe}
\affiliation{University of Pittsburgh, Pittsburgh, PA, 15260, USA}

\author{K.~Wierman}
\affiliation{Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}

\author{Z.~Williams}
\affiliation{University of Texas, Arlington, TX, 76019, USA}

\author{S.~Wolbers}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{T.~Wongjirad}
\affiliation{Tufts University, Medford, MA, 02155, USA}

\author{K.~Woodruff}
\affiliation{New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}

\author{T.~Yang}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{G.~Yarbrough}
\affiliation{University of Tennessee, Knoxville, TN, 37996, USA}

\author{L.~E.~Yates}
\affiliation{Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}

%\author{B.~Yu}    % only for noise paper and signal processing paper #1!
\author{G.~P.~Zeller}
\affiliation{Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}

\author{J.~Zennamo}
\affiliation{University of Chicago, Chicago, IL, 60637, USA}

\author{C.~Zhang}
\affiliation{Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}







\iffalse
% Authors in alphabetical order
%\author[15]{P.~Abratenko}   % only for MCS paper!
\author{C.~Adams}{$^{9}$}
%\author[11]{M.~Alrashed}
\author{R.~An}{$^{10}$}
\author{J.~Anthony$^{3}$}
\author{J.~Asaadi$^{27}$}
\author{M.~Auger$^{1}$}
\author{L.~Bagby$^{8}$}
\author{S.~Balasubramanian$^{31}$}
\author{B.~Baller$^{8}$}
\author{C.~Barnes$^{16}$}
\author{G.~Barr$^{19}$}
\author{M.~Bass$^{19,2}$}
\author{F.~Bay$^{28}$}
\author{A.~Bhat$^{24}$}
\author{K.~Bhattacharya$^{20}$}
\author{M.~Bishai$^{2}$}
\author{A.~Blake$^{12}$}
\author{T.~Bolton$^{11}$}
%\author{B.~Bullard$^{2}$}     % only for noise paper!
\author{L.~Camilleri$^{7}$}
\author{D.~Caratelli$^{7}$}
\author{R.~Castillo~Fernandez$^{8}$}
\author{F.~Cavanna$^{8}$}
\author{G.~Cerati$^{8}$}
\author{H.~Chen$^{2}$}
\author{Y.~Chen$^{1}$}
\author{E.~Church$^{20}$}
\author{D.~Cianci$^{7}$}
\author{E.~Cohen$^{25}$}
\author{G.~H.~Collin$^{15}$}
\author{J.~M.~Conrad$^{15}$}
\author{M.~Convery$^{23}$}
\author{L.~Cooper-Troendle$^{31}$}
\author{J.~I.~Crespo-Anad\'{o}n$^{7}$}
%\author{G.~De~Geronimo$^{2}$}   % only for noise paper!
\author{M.~Del~Tutto$^{19}$}
\author{D.~Devitt$^{12}$}
\author{A.~Diaz$^{15}$}
\author{S.~Dytman$^{21}$}
\author{B.~Eberly$^{23}$}
\author{A.~Ereditato$^{1}$}
\author{L.~Escudero Sanchez$^{3}$}
\author{J.~Esquivel$^{24}$}
\author{J.~Evans$^{14}$}
\author{A.~A.~Fadeeva$^{7}$}
\author{B.~T.~Fleming$^{31}$}
\author{W.~Foreman$^{4}$}
\author{A.~P.~Furmanski$^{14}$}
\author{D.~Garcia-Gamez$^{14}$}
\author{G.~T.~Garvey$^{13}$}
\author{V.~Genty$^{7}$}
\author{D.~Goeldi$^{1}$}
\author{S.~Gollapinni$^{26}$}
\author{E.~Gramellini$^{31}$}
\author{H.~Greenlee$^{8}$}
\author{R.~Grosso$^{5}$}
\author{R.~Guenette$^{19,9}$}
\author{P.~Guzowski$^{14}$}
\author{A.~Hackenburg$^{31}$}
\author{P.~Hamilton$^{24}$}
\author{O.~Hen$^{15}$}
\author{J.~Hewes$^{14}$}
\author{C.~Hill$^{14}$}
\author{J.~Ho$^{4}$}
\author{G.~Horton-Smith$^{11}$}
\author{A.~Hourlier$^{15}$}
\author{E.-C.~Huang$^{13}$}
\author{C.~James$^{8}$}
\author{J.~Jan~de~Vries$^{3}$}
\author{L.~Jiang$^{21}$}
\author{R.~A.~Johnson$^{5}$}
\author{J.~Joshi$^{2}$}
\author{H.~Jostlein$^{8}$}
\author{Y.-J.~Jwa$^{7}$}
\author{D.~Kaleko$^{7}$}
%\author{L.~N.~Kalousis\note{now at: Vrije Universiteit Brussel, 1050 Ixelles, Belgium}} % only for MCS and MuCS papers!
\author{G.~Karagiorgi$^{7}$}
\author{W.~Ketchum$^{8}$}
\author{B.~Kirby$^{2}$}
\author{M.~Kirby$^{8}$}
\author{T.~Kobilarcik$^{8}$}
\author{I.~Kreslo$^{1}$}
%\author{G.~Lange$^{30}$}    % only for MuCS paper!
%\author{S.~Li$^{2}$}   % only for noise paper!
\author{Y.~Li$^{2}$}
\author{A.~Lister$^{12}$}
\author{B.~R.~Littlejohn$^{10}$}
\author{S.~Lockwitz$^{8}$}
\author{D.~Lorca$^{1}$}
\author{W.~C.~Louis$^{13}$}
\author{M.~Luethi$^{1}$}
\author{B.~Lundberg$^{8}$}
\author{X.~Luo$^{31}$}
\author{A.~Marchionni$^{8}$}
\author{S.~Marcocci$^{8}$}
\author{C.~Mariani$^{30}$}
\author{J.~Marshall$^{3}$}
\author{D.~A.~Martinez~Caicedo$^{10}$}
\author{A.~Mastbaum$^{4}$}
\author{V.~Meddage$^{11}$}
\author{T.~Miceli$^{17}$}
\author{G.~B.~Mills$^{13}$}
\author{A.~Mogan$^{26}$}
\author{J.~Moon$^{15}$}
\author{M.~Mooney$^{2,6}$}
\author{C.~D.~Moore$^{8}$}
\author{J.~Mousseau$^{16}$}
\author{M.~Murphy$^{30}$}
\author{R.~Murrells$^{14}$}
\author{D.~Naples$^{21}$}
\author{P.~Nienaber$^{22}$}
\author{J.~Nowak$^{12}$}
\author{O.~Palamara$^{8}$}
\author{V.~Pandey$^{30}$}
\author{V.~Paolone$^{21}$}
\author{A.~Papadopoulou$^{15}$}
\author{V.~Papavassiliou$^{17}$}
\author{S.~F.~Pate$^{17}$}
\author{Z.~Pavlovic$^{8}$}
%\author{R.~Pelkey$^{30}$}    % only for MuCS paper!
\author{E.~Piasetzky$^{25}$}
\author{D.~Porzio$^{14}$}
\author{G.~Pulliam$^{24}$}
\author{X.~Qian$^{2}$}
\author{J.~L.~Raaf$^{8}$}
%\author{V.~Radeka$^{2}$}   % only for noise paper, signal processing paper #1
\author{A.~Rafique$^{11}$} \thanks{Corresponding author}\email[Email: ]{aleena@ksu.edu}
%\author{S.~Rescia$^{2}$}   % only for noise paper!
\author{L.~Rochester$^{23}$}
\author{M.~Ross-Lonergan$^{7}$}
\author{C.~Rudolf~von~Rohr$^{1}$}
\author{B.~Russell$^{31}$}
\author{D.~W.~Schmitz$^{4}$}
\author{A.~Schukraft$^{8}$}
\author{W.~Seligman$^{7}$}
\author{M.~H.~Shaevitz$^{7}$}
\author{J.~Sinclair$^{1}$}
\author{A.~Smith$^{3}$}
\author{E.~L.~Snider$^{8}$}
\author{M.~Soderberg$^{24}$}
\author{S.~S{\"o}ldner-Rembold$^{14}$}
\author{S.~R.~Soleti$^{19}$}
\author{P.~Spentzouris$^{8}$}
\author{J.~Spitz$^{16}$}
\author{J.~St.~John$^{5,8}$}
\author{T.~Strauss$^{8}$}
\author{K.~Sutton$^{7}$}
\author{S.~Sword-Fehlberg$^{17}$}
\author{A.~M.~Szelc$^{14}$}
\author{N.~Tagg$^{18}$}
\author{W.~Tang$^{26}$}
\author{K.~Terao$^{7,23}$}
\author{M.~Thomson$^{3}$}
%\author{C.~Thorn$^{2}$}  % only for noise paper and signal processing paper #1
\author{M.~Toups$^{8}$}
\author{Y.-T.~Tsai$^{23}$}
\author{S.~Tufanli$^{31}$}
\author{T.~Usher$^{23}$}
\author{W.~Van~De~Pontseele$^{19}$}
\author{R.~G.~Van~de~Water$^{13}$}
\author{B.~Viren$^{2}$}
\author{M.~Weber$^{1}$}
\author{H.~Wei$^{2}$}
\author{D.~A.~Wickremasinghe$^{21}$}
\author{K.~Wierman$^{20}$}
\author{Z.~Williams$^{27}$}
\author{S.~Wolbers$^{8}$}
\author{T.~Wongjirad$^{15,29}$}
\author{K.~Woodruff$^{17}$}
\author{T.~Yang$^{8}$}
\author{G.~Yarbrough$^{26}$}
\author{L.~Yates$^{15}$}
%\author{B.~Yu$^{2}$}    % only for noise paper and signal processing paper #1!
\author{G.~P.~Zeller$^{8}$}
\author{J.~Zennamo$^{4}$}
\author{C.~Zhang$^{2}$}

% Institutions in alphabetical order
\affiliation{$^{1}$Universit{\"a}t Bern, Bern CH-3012, Switzerland}
\affiliation{$^{2}$Brookhaven National Laboratory (BNL), Upton, NY, 11973, USA}
\affiliation{$^{3}$University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\affiliation{$^{4}$University of Chicago, Chicago, IL, 60637, USA}
\affiliation{$^{5}$University of Cincinnati, Cincinnati, OH, 45221, USA}
\affiliation{$^{6}$Colorado State University, Fort Collins, CO, 80523, USA}
\affiliation{$^{7}$Columbia University, New York, NY, 10027, USA}
\affiliation{$^{8}$Fermi National Accelerator Laboratory (FNAL), Batavia, IL 60510, USA}
\affiliation{$^{9}$Harvard University, Cambridge, MA 02138, USA}
\affiliation{$^{10}$Illinois Institute of Technology (IIT), Chicago, IL 60616, USA}
\affiliation{$^{11}$Kansas State University (KSU), Manhattan, KS, 66506, USA}
\affiliation{$^{12}$Lancaster University, Lancaster LA1 4YW, United Kingdom}
\affiliation{$^{13}$Los Alamos National Laboratory (LANL), Los Alamos, NM, 87545, USA}
\affiliation{$^{14}$The University of Manchester, Manchester M13 9PL, United Kingdom}
\affiliation{$^{15}$Massachusetts Institute of Technology (MIT), Cambridge, MA, 02139, USA}
\affiliation{$^{16}$University of Michigan, Ann Arbor, MI, 48109, USA}
\affiliation{$^{17}$New Mexico State University (NMSU), Las Cruces, NM, 88003, USA}
\affiliation{$^{18}$Otterbein University, Westerville, OH, 43081, USA}
\affiliation{$^{19}$University of Oxford, Oxford OX1 3RH, United Kingdom}
\affiliation{$^{20}$Pacific Northwest National Laboratory (PNNL), Richland, WA, 99352, USA}
\affiliation{$^{21}$University of Pittsburgh, Pittsburgh, PA, 15260, USA}
\affiliation{$^{22}$Saint Mary's University of Minnesota, Winona, MN, 55987, USA}
\affiliation{$^{23}$SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
\affiliation{$^{24}$Syracuse University, Syracuse, NY, 13244, USA}
\affiliation{$^{25}$Tel Aviv University, Tel Aviv, Israel, 69978}
\affiliation{$^{26}$University of Tennessee, Knoxville, TN, 37996, USA}
\affiliation{$^{27}$University of Texas, Arlington, TX, 76019, USA}
\affiliation{$^{28}$TUBITAK Space Technologies Research Institute, METU Campus, TR-06800, Ankara, Turkey}
\affiliation{$^{29}$Tufts University, Medford, MA, 02155, USA}
\affiliation{$^{30}$Center for Neutrino Physics, Virginia Tech, Blacksburg, VA, 24061, USA}
\affiliation{$^{31}$Yale University, New Haven, CT, 06520, USA}
\fi


%\end{document}
